Tiny Classifier Circuits: Evolving Accelerators for Tabular Data

A typical machine learning (ML) development cycle for edge computing is to maximise the performance during model training and then minimise the memory/area footprint of the trained model for deployment on edge devices targeting CPUs, GPUs, microcontrollers, or custom hardware accelerators. This paper proposes a methodology for automatically generating predictor circuits for classification of tabular data with comparable prediction performance to conventional ML techniques while using substantially fewer hardware resources and power. The proposed methodology uses an evolutionary algorithm to search over the space of logic gates and automatically generates a classifier circuit with maximised training prediction accuracy. Classifier circuits are so tiny (i.e., consisting of no more than 300 logic gates) that they are called "Tiny Classifier" circuits, and can efficiently be implemented in ASIC or on an FPGA. We empirically evaluate the automatic Tiny Classifier circuit generation methodology or "Auto Tiny Classifiers" on a wide range of tabular datasets, and compare it against conventional ML techniques such as Amazon's AutoGluon, Google's TabNet and a neural search over Multi-Layer Perceptrons. Despite Tiny Classifiers being constrained to a few hundred logic gates, we observe no statistically significant difference in prediction performance in comparison to the best-performing ML baseline. When synthesised as a Silicon chip, Tiny Classifiers use 8-18x less area and 4-8x less power. When implemented as an ultra-low cost chip on a flexible substrate (i.e., FlexIC), they occupy 10-75x less area and consume 13-75x less power compared to the most hardware-efficient ML baseline. On an FPGA, Tiny Classifiers consume 3-11x fewer resources.

==> src/deploy_to_fpgas.tex <==
To evaluate the classifier circuits we deploy them as accelerators on a System-on-Chip with integrated FPGA resources (e.g.\ Xilinx Zynq family of platforms). This section presents the synthesized RTL within a software/hardware system targeting Xilinx platforms and we discuss the tradeoffs and the design decisions for the development of the tiny classifier circuits as custom inference engines on FPGAs.

The RTL is generated using High-Level Synthesis tools from Xilinx \cite{xilinx_hls}. The Xilinx SDSoC is the state-of-the-art environment for designing software/hardware targeting the Zynq  platforms \cite{xilinx_sdsoc_env_user} \cite{xilinx_sdsoc_prog_guide}.

This environment produces a complete software/hardware solution for a target platform where the designers develop at the same time the software part along with a C/C++ implementation of the accelerated function which later will be compiled by High-Level Synthesis (HLS). For our work, we develop an application which executes on the processing system (PS) part of the target platform and is able to orchestrate the dataset and handle the calls to the hardware accelerator placed on the Programmable Logic (PL) part.

The classifier circuits are implemented as functions in C/C++ to help the HLS process. The  C/C++ functions use loops to iterate through the test inference data of the dataset, call the predictor functions and perform `classifications'. Each iteration of the loop processes the features of one inference, calls the classifier circuit function and then places the prediction to the output buffer. We choose this strategy mainly because to benefit from the HLS directives \texttt{\#pragma HLS PIPELINE} and \texttt{\#pragma HLS UNROLL}. We use these directives also to balance the throughput/latency of the design with respect to the available resources of the target platform.

Furthermore, we can progressively optimize the design by finding and mapping identical classifier circuit blocks (Figure \ref{fig:parallel_predictors}).  Basically the tiny classifier circuits can be thought as a set of circuit building blocks along with logic to input data and process inferences in parallel.

\begin{figure}[tbh] 
    \centering
    \includegraphics[scale=0.5]{figures/scale_up.pdf}
    \caption{An overview of the programmable accelerator with High-Level-Synthesis. The Processing system part executes the software application which splits the test data into groups (a set of test inferences). Each group can be processed in parallel or sequentially (user-defined parameter).}
    \label{fig:the_soc_implementation}
\end{figure}

The actual design of the accelerator can be split into two main levels. In level one, we handle the function calls to the classifier circuit block(s). At this level, there are four main loops which iterate through the inference group with each loop to iterate on a chunk of eight inferences. The loop body can execute up to 8 parallel inferences in one iteration of the parent loop. The loop body consists of function calls to the second level of loops along with some functions which are responsible to pack and place the predictions back to the local output buffers. The actual predictor circuit blocks are placed in level two. The mapped accelerator uses two identical classifier circuit blocks at this level. These blocks are called in parallel from the loop iterations of level one, and for every iteration, each of the predictor circuit function performs four predictions. We decide to execute the loops in level one sequentially. Each loop body calls the classifier circuit function blocks. This approach offers the ability to use \texttt{\#pragma} directives at various granularity levels and keep the resources low.

Figure \ref{fig:the_soc_implementation} shows the breakdown of an input dataset with 128 inferences. We split the dataset into groups of 32 inferences. Each group can be processed in parallel or sequentially (sequential group-after-group processing). Obviously the parallel version can be translated to a dramatically increase of resources. For the purposes of this work, we explore the sequential version as we target on resource-limited implementations.

==> src/discussion.tex <==
In this work, we have focused on the application of GBGP to learning boolean circuits for classifying tabular data. However, the approach is not in principle limited to tabular data alone. Work on recurrent GBGP \cite{turner2014recurrent} and in particular its application to stateful digital circuits \cite[Ch.~7]{atkinson2019thesis} implies the general applicability of the approach to time-series data. Additional work on GBGP for the synthesis of image filters \cite{slany2007fitness,sekanina2011image} also alludes to the possible application to image-structured data. However, each of these data domains is a significant research question in its own right, which we consider beyond the scope of the initial steps taken here towards GBGP-based ML operating directly at the circuit level. Future work should therefore investigate the extension of the proposed approach to time-series and image-based data, using this literature as a starting point. With such extensions, it would then clearly be of value to perform an extensive empirical analysis similar to that studied here, investigating the both the predictive performance and hardware cost in comparison to SOTA ML techniques. Given the existing literature on the successful evolution of stateful boolean circuits, we hypothesise that similar resource advantages may be obtained in the time-series domain, e.g. in application to speech/audio, forecasting and signal processing.

==> src/evolving_graphs_by_graph_programming.tex <==
While there are a variety of available graph-based genetic programming approaches, we follow existing empirical evidence of the high efficiency of the default instantiation of Evolving Graphs by Graph Programming (EGGP) %\cite{atkinson2019thesis} we should bring it back in camera ready version
for circuit synthesis tasks \cite{atkinson2018evolving,sotto2020study,franccoso2021graph}.  

\subsection{Evolutionary Algorithm}

In this work, we follow the consensus of using the simple $1+\lambda$ evolutionary technique for graph-based genetic programming \cite{miller2019cartesian},  and particularly for circuit synthesis  -- a practice reinforced by recent empirical experiments \cite{sotto2020study,franccoso2021graph}. The algorithm consists of the following steps:

\begin{enumerate}
    \item Generate a random initial parent solution $S$, and evaluate its fitness $f_S$.
    \item While not terminated do:
    \begin{enumerate}
        \item Generate $\lambda$ children $C_1 \dots C_\lambda$ by mutating $S$.
        \item Evaluate the childrens' fitness values $f_1 \dots f_\lambda$.
        \item If any child $C_i$ has $f_i \ge f_S$, then replace the parent $S = C_i$, $f_S = f_i$. Where multiple children satisfy this condition, the child with the highest fitness is chosen, and tie-breaks are determined at random.
    \end{enumerate}
\end{enumerate}

The presence of the $\ge$ operator in the selection of a new parent, rather than just $>$, plays a pivotal role in the performance of the algorithm. In allowing the parent to be replaced by a child with equal fitness, the algorithm mimics the neutral drift of DNA as described in \cite{kimura1983neutral}. This allows the algorithm to undergo a `random walk' in the space of equivalent solutions to the best solution so-far, exposing the algorithm to new neighbourhoods of possible children and thereby allowing it to escape local optima. This simple modification yields significant performance gains in practice \cite{yu2001neutrality, yu2002finding,turner2015neutral} and may be augmented for further gains \cite{atkinson2019evolving,atkinson2020horizontal,downing2006neutrality,turner2015neutral}, although we do not use these extensions in this work. 

\subsection{Solution Representation}

In EGGP, functional programs such as digital circuits are represented as graphs consisting of:

\begin{itemize}
    \item A set of input nodes $V_I$, each node of which uniquely representing an input to the program.
    \item A set of function nodes $V_F$, each node of which representing a specific function applied to its inputs.
    \item A set of output nodes $V_O$, each node of which uniquely representing an output of the program. 
    \item A set of edges $E$ connecting function nodes and output nodes to their respective inputs.
\end{itemize}

While in general the edges of each node are ordered so that they appropriately handle commutative functions \cite{atkinson2018evolving}, in this case all considered functions are symmetric and this is not a practical issue for consideration.

A crucial property of the EGGP representation is that function nodes need not be `active'. If there exists no path from a function node to an output node, then that node has no semantic meaning in the graph. This inactive material can be freely mutated to provide a direct mechanism for neutral drift. Figure \ref{fig:example_ind} shows an example EGGP solution with two inputs and two outputs. 

\begin{figure}
    \centering
    \input{isca2021-latex-template/figures/example_graph.tikz}
    \caption{An example 2-input, 2-output EGGP individual. Nodes $i_1, i_2$ are input nodes, and nodes $o_1, o_2$ are output nodes. Every other node is a function node computing a binary operation on its inputs indicating by its outgoing edges. Inactive material which does not contribute to the semantics of the graph is shown in grey.}
    \label{fig:example_ind}
\end{figure}

\subsection{Genetic Operators}

When using the $1+\lambda$ evolutionary technique there are two main forms of genetic operator; initialisation and mutation. This section details these operators for the EGGP algorithm.

\subsubsection{Initialisation}

Initialisation in EGGP follows the same methodology as that of cartesian genetic programming \cite{miller2008cartesian}. The initialisation is parameterised by the number of function nodes $n$, and the set of possible functions $F$. First, the $I$ input nodes $i_1 \dots i_I$ are created. Then for each $i \in 1 \dots n$, a function node $v_i$ is created and associated with a function chosen uniformly at random from $F$. $v_i$ is then connected uniformly at random to existing nodes $i_1 \dots i_I, v_1 \dots v_{i-1}$ until its degree matches the number of expected inputs to $f$. Finally, the $O$ output nodes $o_1 \dots o_O$ are created, and each is connected uniformly at random to a single node in $i_1 \dots i_I, v_1 \dots v_n$. The hyper-parameter $n$ determines the overall size of the graphs throughout the duration of the evolutionary run.

\subsubsection{Mutation}

Mutation on solutions in EGGP is performed via point mutations drawn from binomial distributions. The mutation rate $p$ parameterises the two binomial distributions $B(n, p)$ and $B(E, p)$ describing mutations of the functions nodes and edges, respectively. With $m_n \sim B(n, p)$ and $m_e \sim B(E, p)$ as the number of node and edge mutations to apply to the graph, the total $m_n + m_e$ mutations are applied in a random shuffled order, where;

\begin{itemize}
    \item For node mutations, a random function node $v \in V_f$ is chosen, and its associated function $f$ is replaced with $f' \in F, f' \neq f$ chosen uniformly at random. As the functions used here are symmetric and of the same arity, there is no need for input shuffling or connection modification procedures as described in \cite{atkinson2019evolving}.
    \item For edge mutations, a random edge $e \in E$ is chosen, where $s$ is the source of $e$ and $t$ is the target of $e$. The edge is redirected such that its new target $v \in V_I \bigcup V_F$ is chosen uniformly at random where the following conditions hold:
    \begin{itemize}
        \item There is no path $v \rightarrow s$ as this would introduce a cycle.
        \item $v \neq t$ as this would not introduce any perturbation of the solution. In the special (very rare) case that the number of inputs $I = 1$ and there is only a single node $t = i_1$ satisfying the first condition, the mutation is abandoned.
    \end{itemize}
\end{itemize}


\subsection{Fitness}

For a circuit C, primary fitness function $\rho$ (e.g. accuracy or balanced accuracy) and secondary fitness function X, a regularised fitness function is constructed:

\begin{equation}
 R(C) = a*\rho(C)-(1-a)*X(C)
\end{equation}
where \textit{a} is a tunable parameter controlling how much the secondary fitness function influences the evolutionary process. Possible secondary fitness functions include:
\begin{itemize}
    \item Number of gates (regularising for size/complexity).
    \item Number of NAND-2 equivalent gates (regularising for power consumption).
    \item  How vulnerable the circuit is to ‘stuck-at’ errors (regularising for fault tolerance). 
\end{itemize}

Our tool chain supports all of the above secondary fitness functions, although in the experiments presented in this paper we consider only the primary fitness function $\rho$, which is the balanced accuracy, e.g. $a=1$. Additionally, the training data is split 50/50, with the latter half reserved for validation with the highest performing solution on the validation data returned as the final predictive classifier.

\subsection{Termination}

In this setting, where the theoretical perfect accuracy of $100\%$ may never be achieved, we require a termination condition. We use a simple model, whereby if the validation fitness (computed on the reserved 50\% validation data) has not improved by at least $\gamma$ within $\kappa$ generations, the algorithm terminates and returns the best discovered solution with respect to the validation data.

\subsection{Hyperparameters}

The hyperparameters of EGGP, and their default settings used in this paper, are therefore;

\begin{itemize}
    \item The number of children per generation, $\lambda = 4$.
    \item The number of function nodes at initialisation, $n = 50$.
    \item The mutation rate, $p=\frac{1}{50}$.
    \item The function set from which solutions may be constructed, $F = \{\texttt{and}, \texttt{or}, \texttt{nand}, \texttt{nor}\}$.
    \item The termination threshold $\gamma = 0.01$.
    \item The corresponding window of generations to achieve that threshold and terminate, $\kappa = 300$.
\end{itemize}
